High Dimensional Data Enrichment: Interpretable, Fast, and Data-Efficient

We consider the problem of multi-task learning in the high dimensional setting. In particular, we introduce an estimator and investigate its statistical and computational properties for the problem of multiple connected linear regressions known as Data Enrichment/Sharing. The between-tasks connections are captured by a cross-tasks \emph{common parameter}, which gets refined by per-task \emph{individual parameters}. Any convex function, e.g., norm, can characterize the structure of both common and individual parameters. We delineate the sample complexity of our estimator and provide a high probability non-asymptotic bound for estimation error of all parameters under a geometric condition. We show that the recovery of the common parameter benefits from \emph{all} of the pooled samples. We propose an iterative estimation algorithm with a geometric convergence rate and supplement our theoretical analysis with experiments on synthetic data. Overall, we present a first thorough statistical and computational analysis of inference in the data-sharing model.

==> sec/proofs.tex <==
%\newpage 
%\onecolumn
\section{Proofs of Theorems}
\label{sec:dsproofs}
Here, we present proof of Proposition \ref{prop:super} and  full proof for Theorem \ref{theo:step} and each lemma used during the proofs of theorems. %To avoid cluttering, during our proofs, we state some needed results as lemmas and provide their proof in the next Section \ref{sec:lemmas}. 
\subsection{Proof of Proposition \ref{prop:super}}
\begin{IEEEproof}
	Consider only one group for regression in isolation. 
	Note that $\y_g = \X_g (\bbeta _g^* + \bbeta _0^*) + \w_g$ is a superposition model and as shown in \cite{guba16} the sample complexity required for the RE condition and subsequently recovering $\bbeta _0^*$ and $\bbeta _g^*$ is $n_g  \geq c(\max(\omega(\cA_0), \omega(\cA_g) ) + \sqrt{\log 2})^2$.
\end{IEEEproof} 

\subsection{Proof of Theorem \ref{theo:step}}
\label{twolems}
	Now we rewrite the same analysis using the tail bounds for the coefficients to clarify the probabilities. 	
	To simplify the notation, we define the following functions of $\tau$:
	\be \nr 
	r_{g1}(\tau) &\triangleq& \frac{1}{2}  \left[\left(1 - \frac{1}{a_g} \right) + \sqrt{2} c_g\frac{2 \omega(\cA_g) + \tau}{a_g \sqrt{n_g}} \right],~\forall g \in [G_+]
	\\ \nr 
	r_{g2}(\tau) &\triangleq& \frac{1}{a_g}  \left(1 + c_{0g}\frac{\omega(\cA_0)+\omega(\cA_g) + \tau}{\sqrt{n_g}} \right),~\forall g \in [G]
	\\ \nr
	r_0(\tau) &\triangleq& r_{01}(\tau)  + \sum_{g=1}^{G} \sqrt{\frac{n_g}{n}} r_{g2}(\tau)
	\\ \nr 
	r_g(\tau) &\triangleq&  r_{g1}(\tau)+ \sqrt{\frac{n_g}{n}} \frac{a_g}{a_0} r_{g2}(\tau),~\forall g \in [G]
	\\ \label{rtau} 
	r(\tau) &\triangleq&  \max_{g \in [G_+] }r_g(\tau)
	\ee
	All of which are computed using $a_g$s specified in the proof sketch of Section \ref{proofsketch}. Basically $r(\tau)$ is an instantiation of an high probability upper bound of the $\rho$ defined in Theorem \ref{theo:iter}.
	We are interested in upper bounding the following probability:
	{\small \begin{align} 
	\label{part1} 
	& \pr \left(\sum_{g=0}^{G} \sqrt{\frac{n_g}{n}} \norm{\ddelta_g^{(t+1)}}{2} \geq  r(\tau)^t \sum_{g=0}^{G}\sqrt{\frac{n_g}{n}} \norm{\bbeta ^*_g}{2}   + \frac{C (G+1)\sqrt{(2k_w^2 + 1)k_x^2}}{(1 - r(\tau))\sqrt{n}} (\max_{g \in [G_+]} \omega(\cA_g) + \tau) \right)
	\\ \nr 
	&\leq 
	\pr \Bigg(\rho^t \sum_{g=0}^{G}\sqrt{\frac{n_g}{n}}\norm{\bbeta ^*_g}{2}   + \frac{1 - \rho^t}{1 -  \rho}   \sum_{g=0}^{G} \sqrt{\frac{n_g}{n}} \eta_g\left(\mu_g\right) \norm{\w_g}{2} \geq 
%	\\ \nr 
	r(\tau)^t \sum_{g=0}^{G} \sqrt{\frac{n_g}{n}}\norm{\bbeta ^*_g}{2}   + \frac{C(G+1)\sqrt{(2k_w^2 + 1)k_x^2}}{(1 - r(\tau))\sqrt{n}} (\max_{g \in [G_+]} \omega(\cA_g) + \tau) \Bigg) 
	\\ \nr 
	&\leq  \pr \left( \rho \geq r(\tau) \right)
%	\\ \nr %\label{eq:bigbound} 
	+ \pr \left( \frac{1}{1 -  \rho}  \sum_{g=0}^{G} \sqrt{n_g} \eta_g\left(\mu_g\right) \norm{\w_g}{2} 
	\geq \frac{C(G+1)\sqrt{(2k_w^2 + 1)k_x^2}}{(1 - r(\tau))} (\max_{g \in [G_+]} \omega(\cA_g) + \tau) \right)
	\end{align}}
	where the first inequality comes from the deterministic bound of Theorem \ref{theo:iter} and the second one is based on the law of total probability.	
	
	We first focus on bounding the first term $\pr \left( \rho \geq r(\tau) \right)$:
	{\small \begin{align}	
	\nr 	
	\pr \left( \rho \geq r(\tau) \right)	
	=& \pr \left( \max\left(\rho_0\left(\mu_0\right) + \sum_{g=1}^{G} \sqrt{\frac{n_g}{n}} \phi_g\left(\mu_g\right), \max_{g \in [G]} \rho_g\left(\mu_g\right) + \sqrt{\frac{n}{n_g}} \frac{\mu_0}{\mu_g}\phi_g\left(\mu_g\right)\right) \geq \max_{g \in [G_+] } r(\tau)  \right) 
	\\ \nr 
	(\text{Union Bound}) \leq& \pr \left(\rho_0\left(\mu_0 \right) + \sum_{g=1}^{G} \sqrt{\frac{n_g}{n}} \phi_g\left(\mu_g\right) \geq r_0  \right)   + \sum_{g=1}^{G} \pr \left( \rho_g\left(\mu_g\right) + \sqrt{\frac{n}{n_g}} \frac{\mu_0}{\mu_g}\phi_g\left(\mu_g\right) \geq r_g  \right)
	\\ \nr 
	\leq& \pr \left(\rho_0\left(\mu_0 \right) \geq r_{01} \right) + \sum_{g=1}^{G} \pr\left( \phi_g\left(\mu_g\right) \geq r_{g2}  \right)   + \sum_{g=1}^{G} \left[\pr \left( \rho_g\left(\mu_g\right) \geq r_{g1} \right) + \pr \left(\phi_g\left(\mu_g\right) \geq r_{g2}  \right)\right]
	\\ \nr 
	\leq& \sum_{g=0}^{G} \pr \left( \rho_g\left(\mu_g\right) \geq r_{g1} \right)  + 2\sum_{g=1}^{G} \pr\left( \phi_g\left(\mu_g\right) \geq r_{g2}  \right)   
	\\ \nr 	
	\leq& \sum_{g=0}^{G} 2 \exp\left( -\gamma_g (\omega(\cA_g) + \tau)^2  \right)  + 2\sum_{g=1}^{G} 2\exp\left( -\gamma_g (\omega(\cA_g) + \tau)^2  \right)      
	\\ \nr 	
	(\gamma = \min_{g \in [G_+]} \gamma_g) \leq& 2(G+1)\exp\left( -\gamma \min_{g \in [G_+]} (\omega(\cA_g) + \tau)^2  \right)  + 4 G \exp\left( -\gamma \min_{g \in [G]} (\omega(\cA_g) + \tau)^2  \right)      
	\\  \label{eq:part1} 
	\leq& 6 (G+1)\exp\left( -\gamma \min_{g \in [G_+]} (\omega(\cA_g) + \tau)^2  \right)  
	\end{align}	}
	Now we focus on bounding the second term:
	{\small\bea
	\nr 	
	& \pr \left( \frac{1}{1 - \rho}  \sum_{g=0}^{G} \sqrt{n_g} \eta_g\left(\mu_g \right) \norm{\w_g}{2} 
	\geq \frac{C(G+1)\sqrt{(2k_w^2 + 1)k_x^2}}{(1 - r(\tau))} (\max_{g \in [G_+]} \omega(\cA_g) + \tau) \right)
	\\ \nr 
	&\hspace*{5.5cm}\leq \pr \left( \frac{1}{1 - \rho}  \sum_{g=0}^{G} \sqrt{n_g} \eta_g\left(\mu_g \right) \norm{\w_g}{2} 
	\geq \frac{C}{(1 - r(\tau))} \sum_{g=0}^{G} \sqrt{(2k_w^2 + 1)k_x^2} (\max_{g \in [G_+]} \omega(\cA_g) + \tau) \right) 
	\\ \nr 
	&\hspace*{5.5cm}\leq \pr \left( \sum_{g=0}^{G} \sqrt{n_g} \eta_g\left(\mu_g \right) \norm{\w_g}{2} \geq \sum_{g=0}^{G} c_g \sqrt{(2k_w^2 + 1)k_x^2} (\max_{g \in [G_+]} \omega(\cA_g) + \tau) \right) 
	+ \pr \left( \rho \geq r(\tau) \right)	
	\\ \label{eq:part2}
	&\hspace*{5.5cm}\leq \sum_{g=0}^{G} \pr \left(   \sqrt{n_g} \eta_g\left(\mu_g \right) \norm{\w_g}{2} \geq c_g \sqrt{(2k_w^2 + 1)k_x^2} (\max_{g \in [G_+]} \omega(\cA_g) + \tau) \right) 
	+ \pr \left( \rho \geq r(\tau) \right)		
	\eea}
	Focusing on the first term, since $\eta_g(\frac{1}{a_g n_g}) = \frac{1}{a_g n_g} \sup_{\v \in \cB_g} \v^T \X_g^T \frac{\w_g}{\norm{\w_g}{2}}, \forall g \in [G]$: 
	\bea
	\label{eq:part3}
	&\pr \left( \norm{\w_g}{2} \sup_{\v \in \cB_g} \v^T \X_g^T \frac{\w_g}{\norm{\w_g}{2}}   \geq a_g c_g \sqrt{(2k_w^2 + 1)k_x^2 n_g} (\max_{g \in [G_+]} \omega(\cA_g) + \tau)  \right) 
	\\ \nr 
	(a_g \geq 1)&\leq \pr \left( \norm{\w_g}{2} \sup_{\v \in \cB_g} \v^T \X_g^T \frac{\w_g}{\norm{\w_g}{2}}   \geq c_g \sqrt{(2k_w^2 + 1)k_x^2 n_g} (\max_{g \in [G_+]} \omega(\cA_g) + \tau)  \right) 
	\\ \nr 
	(\eqref{eq:omeggg} \text{ and } \eqref{eq:widthbound})&\leq 2\exp(-\nu n_g) + \pi_g \exp(-\tau^2) 
	\\ \nr 
	(\sigma_g = \max(\pi_g, 2)) &\leq \sigma_g \exp(- \min (\nu n_g, \tau^2) )
	\eea	 
	where we used the intermediate form of Lemma \ref{lemm:mainlem} for  $\tau > 0$.
	Putting all of the bounds \eqref{eq:part1}, \eqref{eq:part2}, and \eqref{eq:part3} back as the upper bound of \eqref{part1}:
	
	\be 
	\nr 
	(\pi = \max_{g \in [G] } \pi_g)
	&\leq&2(G+1)\exp(-\nu \min_{g \in [G]} n_g) + \pi (G+1) \exp(-\tau^2) + 
	\\ \nr 
	\quad && 6 (G+1)\exp\left( -\gamma \min_{g \in [G_+]} (\omega(\cA_g) + \tau)^2  \right)
	\\ \nr 	
	(\upsilon  = \max(6, \pi), \zeta  = \min(1, \gamma) )
	&\leq&2\exp(-\nu \min_{g \in [G]} n_g + \log(G+1)) + \upsilon (G+1) \exp(-\zeta \tau^2) 
	\\ \nr 
	(\tau = \epsilon + \sqrt{\log(G+1)}/\zeta)
	&\leq&2\exp(-\nu \min_{g \in [G]} n_g + \log(G+1)) + \upsilon \exp(-\zeta \epsilon^2) 
	\\ \nr 
	(\sigma = \max(2, \upsilon))
	&\leq& \sigma \exp(- \min(\nu \min_{g \in [G]} n_g - \log(G+1), \zeta \epsilon^2) )
	\ee	
 	Note that setting $\tau = \epsilon + \sqrt{\log(G+1)}/\zeta$ increases the sample complexities to the followings:
	\be 
	\nr 
	n > 2 c_0^2 \left(2 \omega(\cA_0) + \sqrt{\log (G+1)}/\zeta + \epsilon\right)^2, \forall g \in [G]: n_g \geq 2c_g^2 (2 \omega(\cA_g) + C\sqrt{\log (G+1)}/\zeta  + \epsilon)^2
	\ee 
	And it also affects step sizes as follows:
	{\small\be
	\nr  
	\mu_0 = \frac{1}{4	n} \times \min_{g \in [G]} \left(1 + c_{0g} \frac{\omega_{0g}+\sqrt{\log (G+1)}/\zeta  + \epsilon}{\sqrt{n_g}}\right)^{-2} , \mu_g =  \frac{1}{2\sqrt{n n_g}} \left(1 + c_{0g}\frac{\omega_{0g}+ \sqrt{\log (G+1)}/\zeta  + \epsilon}{\sqrt{n_g}} \right)^{-1}
	\ee }
	
	
		






%\section{Proofs of Lemmas}
%\label{sec:lemmas}
%Here, we present proofs of each lemma used during the proofs of theorems.
%

\subsection{Proof of Lemma \ref{lemm:shareInc}}
\begin{IEEEproof}
	LHS of \eqref{eq:rhs} is the weighted summation of $\xi_g Q_{2\xi_g}(\ddelta_{0g}) = \norm{\ddelta_{0g}}{2}\xi \pr(|\langle \x, , \ddelta_{0g}/\norm{\ddelta_{0g}}{2} \rangle| > 2\xi) = \norm{\ddelta_{0g}}{2}\xi Q_{2\xi}(\u)$ where $\xi > 0$ and $\u = \ddelta_{0g}/\norm{\ddelta_{0g}}{2}$ is a unit length vector. 
	So we can rewrite the LHS of \eqref{eq:rhs} as:
	\be 
	\nr 
	\sum_{g=1}^G\frac{n_g}{n}\xi_g Q_{2\xi_g}(\ddelta_{0g}) = \sum_{g=1}^G\frac{n_g}{n}\norm{\ddelta_{0} +  \ddelta_{g}}{2}\xi Q_{2\xi}(\u), \quad \u \in \sphere
	\ee 
	With this observation, the lower bound of the Lemma \ref{lemm:shareInc} is a direct consequence of the following two results: 
	\begin{lemma}\label{paley} Let $\u$ be any unit length vector and suppose $\x$ obeys Definition \ref{def:obs}. Then for any $\u$, we have
		\be 
		Q_{2\xi}(\u) \geq \frac{(\alpha - 2\xi)^2}{4ck_x^2}.
		\ee 	
	\end{lemma}
	\begin{lemma} \label{incolem main} Suppose Definition \ref{incodef} holds. Then, we have: 
		\be 
		\sum_{g=1}^G \frac{n_g}{n} \norm{\ddelta_0+\ddelta_g}{2}\geq\frac{\ratio\lamin}{3} \left( G\norm{\ddelta_0}{2} + \sum_{g=1}^G \frac{n_g}{n} \norm{\ddelta_g}{2} \right), \quad \forall g \in [G_+]: \ddelta_g \in \cC_g.
		\ee 
	\end{lemma}	
\end{IEEEproof}



\subsection{Proof of Lemma \ref{lemm:secTerm}}
\begin{IEEEproof}
	\label{sec:proofSecTerm}
	Consider the following soft indicator function which we use in our derivation:
	\be
	\nr  
	\psi_a (s) = 
	\begin{cases}
		0, & |s| \leq a \\
		(|s| - a)/a, & a \leq |s| \leq 2 a \\ 
		1, & 2a < |s| 
	\end{cases}
	\ee 
	\begin{figure}[th!]
		\centering
		\includegraphics[width=.5\textwidth]{./img/funcs.pdf}				
		\caption{$\indic(|s|> 2a) \leq \psi_a (s) \leq \indic(|s|>a)$}
		\label{funcs}
	\end{figure}
	Now using the definition of the marginal tail function we have:
	\be 	
	\nr 
	&&\ex \sup_{\ddelta \in \cH} \sum_{g=1}^{G} \xi_g  \sum_{i=1}^{n_g} \left[Q_{2 \xi_g}(\ddelta_{0g})  - \indic (|\langle \x_{gi}, \ddelta_{0g} \rangle| \geq \xi_g )  \right]
	\\ \nr 
	&=& \ex \sup_{\ddelta \in \cH} \sum_{g=1}^{G} \xi_g  \sum_{i=1}^{n_g} \left[\ex \indic (|\langle \x_{gi}, \ddelta_{0g} \rangle| \geq 2\xi_g )   - \indic (|\langle \x_{gi}, \ddelta_{0g} \rangle| \geq \xi_g )  \right] 
	\\ \nr 
	(\text{Figure \ref{funcs}}) &\leq& 
	\ex \sup_{\ddelta \in \cH} \sum_{g=1}^{G} \xi_g  \sum_{i=1}^{n_g} \left[\ex \psi_{\xi_g }(\langle \x, \ddelta_{0g} \rangle)   - \psi_{\xi_g }(\langle \x_{gi}, \ddelta_{0g} \rangle)   \right] 
	\\ \nr  
	(\text{Symmetrization \cite{Vaart1996-zl}}) &\leq& 
	2 \ex \sup_{\ddelta \in \cH} \sum_{g=1}^{G} \xi_g  \sum_{i=1}^{n_g} \epsilon_{gi} \psi_{\xi_g }(\langle \x_{gi}, \ddelta_{0g} \rangle)
	\\ \nr 
	(\text{Rademacher comparison \cite{Ledoux1991-ix}}) &\leq& 
	2 \ex \sup_{\ddelta \in \cH} \sum_{g=1}^{G} \sum_{i=1}^{n_g} \epsilon_{gi} \langle \x_{gi}, \ddelta_{0g} \rangle
	\ee  
	where $\epsilon_{gi}$ are iid copies of Rademacher random variable which are independent of every other random variables and themselves.

	Now we add back $\frac{1}{n}$ and expand $\ddelta_{0g} = \ddelta_{0} + \ddelta_{g}$. Also, we substitute $\ddelta \in \cH$ constraint with $\ddelta \in \cC$ because $\cH \subseteq \cC$ where $\cC = \{ \ddelta = (\ddelta_0^T, \dots, \ddelta_G^T)^T \Big| \ddelta_g \in \cC_g \}$: 
	
	\be 
	\nr 
	\frac{2}{n} \ex \sup_{\ddelta \in \cC} \sum_{g=1}^{G} \sum_{i=1}^{n_g} \epsilon_{gi} \langle \x_{gi}, \ddelta_{0g} \rangle
	&=& \frac{2}{n} \ex \sup_{\ddelta_0 \in \cC_0} \sum_{i=1}^{n} \epsilon_{i} \langle \x_{i}, \ddelta_{0} \rangle
	+ \frac{2}{n} \ex \sup_{\forall g \in [G]: \ddelta_g \in \cC_g} \sum_{g=1}^{G} \sum_{i=1}^{n_g} \epsilon_{gi} \langle \x_{gi}, \ddelta_{g} \rangle
	\\ \nr 
	&=&
	\frac{2}{\sqrt{n}} \ex \sup_{\ddelta_0 \in \cC_0} \sum_{i=1}^{n} \langle \frac{1}{\sqrt{n}} \epsilon_{i} \x_{i}, \ddelta_{0} \rangle
	+ \frac{2}{\sqrt{n}} \ex \sup_{\forall g \in [G]: \ddelta_g \in \cC_g} \sum_{g=1}^{G}  \sqrt{\frac{n_g}{n}} \sum_{i=1}^{n_g} \langle \frac{1}{\sqrt{n_g}} \epsilon_{gi} \x_{gi}, \ddelta_{g} \rangle
	\\ \nr 
	(n_0 := n, \epsilon_{0i} := \epsilon_0, \x_{0i} := \x_i) &=& \frac{2}{\sqrt{n}} \ex \sup_{\forall g \in [G_+]: \ddelta_g \in \cC_g} \sum_{g=0}^{G}  \sqrt{\frac{n_g}{n}} \sum_{i=1}^{n_g} \langle \frac{1}{\sqrt{n_g}} \epsilon_{gi} \x_{gi}, \ddelta_{g} \rangle
	\\ \nr 
	(\h_{g} := \frac{1}{\sqrt{n_g}} \sum_{i=1}^{n_g} \epsilon_{gi} \x_{gi}) &=& \frac{2}{\sqrt{n}} \ex \sup_{\forall g \in [G_+]: \ddelta_g \in \cC_g} \sum_{g=0}^{G}  \sqrt{\frac{n_g}{n}}  \langle \h_{g}, \ddelta_{g} \rangle
	\\ \nr 
	(\u_g \in \frac{\ddelta_g}{\norm{\ddelta_g}{2}}, \cA_g \in \cC_g \cap \sphere) &\leq& \frac{2}{\sqrt{n}} \ex \sup_{\forall g \in [G_+]: \u_g \in \cA_{g}} \sum_{g=0}^{G}  \sqrt{\frac{n_g}{n}} \langle \h_{g}, \u_{g} \rangle \norm{\ddelta_{g}}{2}
	\\ \nr 
	(\sup \sum < \sum \sup) &\leq& \frac{2}{\sqrt{n}} \sum_{g=0}^{G}  \sqrt{\frac{n_g}{n}} \ex_{\h_{g}} \sup_{\u_g \in \cA_g}  \langle \h_{g}, \u_{g} \rangle \norm{\ddelta_{g}}{2}
	\\ \nr 
	&\leq& \frac{2}{\sqrt{n}} \sum_{g=0}^{G}  \sqrt{\frac{n_g}{n}} c_g k_x \omega(\cA_g) \norm{\ddelta_{g}}{2}
	\ee
	Note that the $\h_{gi}$ is a sub-Gaussian random vector which let us bound the $\ex \sup$ using the Gaussian width \cite{trop15} in the last step. 
\end{IEEEproof}

\subsection{Proof of Lemma \ref{lemm:mainlem}}
\begin{IEEEproof} 
	To avoid cluttering let $h_g(\w_g, \X_g) \triangleq \norm{\w_g}{2} \sup_{\u_g \in \cA_g} \langle \X_g^T \frac{\w_g}{\norm{\w_g}{2}}, \u_g \rangle $ be a random quantity and $e_g(\tau) \triangleq c_g k_x (\omega(\cA_g)+\sqrt{\log (G+1)} + \tau)$, and $s_g \triangleq \sqrt{(2k_w^2 + 1)n_g}$ constants. From the law of total probability, we have:	
	{\small\bea
	\nr 
	\pr\left( h_g(\w_g , \X_g) >  s_g e_g(\tau) \right) 
	=& \pr \left( h_g(\w_g , \X_g) >  s_g e_g(\tau) \Big| \norm{\w_g}{2} > s_g \right) \pr\left(\norm{\w_g}{2} > s_g\right) \\ 
	\nr
	+& \pr \left( h_g(\w_g , \X_g) >  s_g e_g(\tau) \Big| \norm{\w_g}{2} < s_g \right) \pr\left(\norm{\w_g}{2} < s_g\right) \\ 
	\nr 
	\leq& \pr\left(\norm{\w_g}{2} > s_g \right) + \pr \left( \norm{\w_g}{2} \sup_{\u_g \in \cA_g} \langle \X_g^T \frac{\w_g}{\norm{\w_g}{2}}, \u_g \rangle >  s_g e_g(\tau) \Big| \norm{\w_g}{2} < s_g \right) \\
	\nr 
	\leq& \pr\left(\norm{\w_g}{2} > \sqrt{(2k_w^2 + 1)n_g}\right) + \pr \left( \sup_{\u_g \in \cC_g \cap \sphere} \langle \X_g^T \frac{\w_g}{\norm{\w_g}{2}}, \u_g \rangle >  e_g(\tau)  \right) \\
	\label{eq:twoterms} 
	\leq& \pr\left(\norm{\w_g}{2} > \sqrt{(2k_w^2 + 1)n_g}\right) + \sup_{\v \in \sphere}\pr \left( \sup_{\u_g \in \cC_g \cap \sphere} \langle \X_g^T \v , \u_g \rangle >  e_g(\tau)  \right)
	\eea }
	Let's focus on the first term. 
	Since $\w_g$ consists of i.i.d. centered unit-variance sub-Gaussian elements with $\normth{w_{gi}}{\psi_2} < k_w$, $w_{gi}^2$ is sub-exponential with $\normth{\w_{gi}}{\psi_1} < 2k_w^2$. 
	Let's apply the Bernstein’s inequality \cite{boucheron13} to $\norm{\w_g}{2}^2 = \sum_{i=1}^{n_g} \w_{gi}^2$:
	
	\be 
	\nr 
	\pr\left( \big| \norm{\w_g}{2}^2  - \ex\norm{\w_g}{2}^2  \big|  > \tau \right) \leq 
	2 \exp\left(-\nu  \min\left[\frac{\tau^2}{4k_w^4n_g}, \frac{\tau }{2k_w^2}\right]\right) 
	\ee
	We also know that $\ex \norm{\w_g}{2}^2 \leq n_g$ \cite{vershynin2018high} which gives us:
	\be
	\nr 
	\pr\left( \norm{\w_g}{2}  > \sqrt{n_g + \tau } \right) \leq 
	2 \exp\left(-\nu  \min\left[\frac{\tau^2}{4k_w^4n_g}, \frac{\tau }{2k_w^2}\right]\right)
	\ee	
	Finally, we set $\tau = 2k_w^2 n_g$:
	\beq
%	\nr 
	\label{eq:omeggg}
	\pr\left( \norm{\w_g}{2}  > \sqrt{(2k_w^2 + 1)n_g } \right) 
	\leq 2\exp\left(-\nu n_g \right) = \frac{2}{(G+1)} \exp\left(-\nu n_g + \log (G+1)\right)
	\eeq
%	Finally, we set $\tau = 2k_w^2 (n_g + \frac{\log(G+1)}{\nu_g})$:
%	\be
%	\nr 
%	%\label{eq:omeggg}
%	&&\pr\left( \norm{\oomega_g}{2}  > \sqrt{(2k_w^2 + 1) (n_g + \frac{\log(G+1)}{\nu_g}) } \right) 
%	\leq 2\exp\left(-\nu_g \min\left[\frac{\left(n_g + \frac{\log(G+1)}{\nu_g}\right)^2}{n_g}, \left(n_g + \frac{\log(G+1)}{\nu_g}\right) \right] \right) 
%	\\ \nr
%	&\leq& 2\exp\left(-\nu_g \min\left[(n_g + \frac{2\log(G+1)}{v_g} + \frac{\log^2(G+1)}{\nu_g^2 n_g}), (n_g + \frac{\log(G+1)}{\nu_g}) \right] \right) 
%	\\ \nr
%	&\leq& 2\exp\left(-\nu_g n_g - \log(G+1) \right) 
%	\\ \nr
%	&=& \frac{2}{(G+1)} \exp\left(-\nu_g n_g \right)
%	\ee 

	Now we upper bound the second term of \eqref{eq:twoterms}.
	Given any fixed $\v \in \sphere$, $\X_g \v$ is a sub-Gaussian random vector with $\normth{\X_g^T \v}{\psi_2} \leq C_gk_x$ \cite{banerjee14}. 
	From Theorem 9 of \cite{banerjee14} for any $\v \in \sphere$ we have:
	\beq 
	\label{eq:widthbound}
	\pr \left( \sup_{\u_g \in \cA_g} \langle \X_g^T \v , \u_g \rangle >  \upsilon_g C_gk_x \omega(\cA_g) + t  \right)
	\leq \pi_g \exp \left( - \left( \frac{t}{\theta_g C_g k_x \phi_g}\right)^2 \right)
	\eeq 	
	where $\phi_g = \sup_{\u_g \in \cA_g} \norm{\u_g}{2}$ and in our problem $\phi_g = 1$. 
	To simplify we take $c_g  = C_g \max(\upsilon_g, \theta_g)$ and then substitute $t = c_g k_x (\tau + \sqrt{\log (G+1)})$:
	\be 
	\nr 
	\pr \left( \sup_{\u_g \in \cA_g} \langle \X_g^T \v , \u_g \rangle >  c_gk_x \left(\omega(\cA_g) + \sqrt{\log (G+1)} + \tau\right) \right)
	&\leq& \pi_g \exp \left( - \left( \tau + \sqrt{\log (G+1)} \right)^2 \right) \\ 
	\nr 
	&\leq& \pi_g \exp \left( - \log (G+1) - \tau^2 \right) \\ 
	\nr 
	&\leq& \frac{\pi_g}{(G+1)} \exp (-\tau^2)
	\ee 	
	Now we put back results to the original inequality \eqref{eq:twoterms}:
	\be 
	\nr
	&& \pr\left( h_g(\w_g , \X_g) >  \sqrt{(2k_w^2 + 1)n_g} \times c_g k_x \left(\omega(\cA_g)+\sqrt{\log (G+1)} + \tau\right) \right) 
	\\ \nr 
	&\leq& \frac{2}{(G+1)} \exp\left(-\nu n_g + \log (G+1)\right) + \frac{\pi_g}{(G+1)} \exp\left(-\tau^2\right) \\ 
	\nr 
	&\leq& \frac{\sigma_g}{(G+1)} \exp\left(-\min\left[\nu  n_g - \log (G+1), \tau^2\right]\right) 
	\ee 
	where $\sigma_g = \pi_g + 2$.
\end{IEEEproof}

\subsection{Proof of Lemma \ref{lem:recurse}}
\begin{IEEEproof}
	We upper bound the individual error $\norm{\ddelta_g^{(t+1)}}{2}$ and the common one $\norm{\ddelta_0^{(t+1)}}{2}$ in the followings:
	
	\be
	\nr 
	\norm{\ddelta_g^{(t+1)}}{2} &=& \norm{\bbeta _g^{(t+1)} - \bbeta _g^*}{2} \\ \nr  
	&=& \normlr{\Pi_{\Omega_{f_g}} \bigg(\bbeta_g^{(t)} + \mu_g \X_g^T \Big(\y_g - \X_g \big(\bbeta_0^{(t)} + \bbeta_g^{(t)}\big) \Big) \bigg) - \bbeta _g^*}{2} \\ \nr 
	\text{(Lemma 6.3 of \cite{oyrs15})}&=& \normlr{\Pi_{\Omega_{f_g}-\{ \bbeta _g^* \}} \bigg(\bbeta_g^{(t)} + \mu_g \X_g^T \Big(\y_g - \X_g \big(\bbeta_0^{(t)} + \bbeta_g^{(t)}\big) \Big) - \bbeta _g^* \bigg)}{2} \\ \nr 
	&=& \normlr{\Pi_{\cE_g} \bigg(\ddelta_g^{(t)} + \mu_g \X_g^T \Big(\y_g - \X_g \big(\bbeta_0^{(t)} + \bbeta_g^{(t)}\big) - \X_g \big(\bbeta _0^* + \bbeta _g^* \big) + \X_g \big(\bbeta _0^* + \bbeta _g^*\big) \Big) \bigg)}{2} \\ \nr 
	&=& \normlr{\Pi_{\cE_g} \bigg(\ddelta_g^{(t)} + \mu_g \X_g^T \Big(\oomega_g - \X_g \big(\ddelta_0^{(t)}  + \ddelta_g^{(t)}\big) \Big) \bigg)}{2} \\ \nr 
	\text{(Lemma 6.4 of \cite{oyrs15})}&\leq&  \normlr{\Pi_{\cC_g} \bigg(\ddelta_g^{(t)} + \mu_g \X_g^T \Big(\oomega_g - \X_g \big(\ddelta_0^{(t)}  + \ddelta_g^{(t)}\big) \Big) \bigg)}{2} \\ \nr 
	\text{(Lemma 6.2 of \cite{oyrs15})}&\leq&  \sup_{\v \in \cC_g \cap \ball} \v^T \bigg(\ddelta_g^{(t)} + \mu_g \X_g^T \Big(\oomega_g - \X_g \big(\ddelta_0^{(t)}  + \ddelta_g^{(t)}\big) \Big) \bigg) \\ \nr
	(\cB_g =  \cC_g \cap \ball) &=&  \sup_{\v \in \cB_g} \v^T \bigg(\ddelta_g^{(t)} + \mu_g \X_g^T \Big(\oomega_g - \X_g \big(\ddelta_0^{(t)}  + \ddelta_g^{(t)}\big) \Big) \bigg) \\ \nr
	&\leq&  \sup_{\v \in \cB_g} \v^T \big(\I_g - \mu_g \X_g^T \X_g\big) \ddelta_g^{(t)} +  \mu_g \sup_{\v \in \cB_g} \v^T \X_g^T \oomega_g  +  \mu_g \sup_{\v \in \cB_g} -\v^T \X_g^T \X_g \ddelta_0^{(t)}   \\ \nr
	&\leq&  \normlr{\ddelta_g^{(t)}}{2} \sup_{\u, \v \in \cB_g} \v^T \big(\I_g - \mu_g \X_g^T \X_g\big) \u  +  \mu_g \norm{\oomega_g}{2} \sup_{\v \in \cB_g} \v^T \X_g^T \frac{\oomega_g}{\norm{\oomega_g}{2}}  \\ \nr 
	&+&  \mu_g  \norm{\ddelta_0^{(t)} }{2}  \sup_{\v \in \cB_g, \u \in \cB_0} -\v^T \X_g^T \X_g \u \\ \nr   
	&=&  \rho_g(\mu_g)\norm{\ddelta_g^{(t)}}{2}   +   \xi_g(\mu_g) \norm{\oomega_g}{2} +  \phi_g(\mu_g) \norm{\ddelta_0^{(t)}}{2} 
	\ee 
	%	where $\theta_f = 1$ for convex $f$ and $\theta_f = 2$ for the non-convex case. 
	%	Note that the last term is lower bounded by zero. To see this clearly consider the set $\cB_{0g} = \{\ddelta_0 + \ddelta_{g} | \ddelta_0 \in \cC_0, \ddelta_g \in \cC_g, \norm{\ddelta_0 + \ddelta_g}{2} \leq 1\}$ where $\cB_0, \cB_g \subseteq \cB_{0g}$:
	%	\be 
	%	\label{eq:zerolb}
	%	\inf_{\v \in \cB_g, \u \in \cB_0} \v^T \X_g^T \X_g \u &\geq& \inf_{\u \in \cB_{0g}} \norm{\X_g \u}{2}^2 \geq 0
	%	\ee 
	So the final bound becomes:
	\beq 
	\label{eq:optg}
	\norm{\ddelta_g^{(t+1)}}{2} \leq \rho_g(\mu_g)\norm{\ddelta_g^{(t)}}{2}   +  \xi_g(\mu_g) \norm{\oomega_g}{2} + \phi_g(\mu_g) \norm{\ddelta_0^{(t)}}{2} 
	\eeq 	
	Now we upper bound the error of common parameter. Remember common parameter's update:
	$\bbeta _0^{(t+1)} = \Pi_{\Omega_{f_0}} \left(\bbeta_0^{(t)} + \mu_0 \X_0^T   
	\begin{pmatrix}
	(\y_1 - \X_1 (\bbeta_0^{(t)} + \bbeta _1^{(t)}))     \\
	\vdots 	 \\
	(\y_G - \X_G (\bbeta_0^{(t)} + \bbeta _G^{(t)})) 
	\end{pmatrix}\right)$.
	
	\bea 
	\nr 
	\norm{\ddelta_0^{(t+1)}}{2} =& \norm{\bbeta _0^{(t+1)} - \bbeta _0^*}{2} \\ \nr  \\ \nr 
	=& \normlr{\Pi_{\Omega_{f_0}} \bigg(\bbeta_0^{(t)} + \mu_0 \sum_{g = 1}^{G} \X_g^T \Big(\y_g - \X_g (\bbeta_0^{(t)} + \bbeta_g^{(t)}) \Big) \bigg) - \bbeta _0^*}{2} \\ \nr 
	\text{(Lemma 6.3 of \cite{oyrs15})} =& \normlr{\Pi_{\Omega_{f_0}-\{ \bbeta _0^* \}} \bigg(\bbeta_0^{(t)} + \mu_0 \sum_{g = 1}^{G}   \X_g^T \Big(\y_g - \X_g (\bbeta_0^{(t)} + \bbeta_g^{(t)}) \Big) - \bbeta _0^* \bigg)}{2} \\ \nr 
	%		&=& \normlr{\Pi_{\cE_0} \bigg(\ddelta_0^{(t)} + \mu_0 \X_0^T \Big(\y - \X_0 \bbeta_0^{(t)} - \tD \bbeta _{1:g}^{t} - \X_0 \bbeta _0^* - \tD \bbeta _{1:g}^* + \X_0 \bbeta _0^* + \tD \bbeta _{1:g}^*   \Big) \bigg)}{2} \\ \nr 
	%		&=& \normlr{\Pi_{\cE_0} \bigg(\ddelta_0^{(t)} + \mu_0 \X_0^T \Big(\oomega - \X_0 \big( \bbeta_0^{(t)} - \bbeta _0^* \big) - \tD \big( \bbeta _{1:g}^{t} - \bbeta _{1:g}^*  \big) \Big) \bigg)}{2} \\ \nr 
	=& \normlr{\Pi_{\cE_0} \bigg(\ddelta_0^{(t)} + \mu_0\sum_{g = 1}^{G}   \X_g^T \Big(\y_g - \X_g (\bbeta_0^{(t)} + \bbeta_g^{(t)}) \Big)}{2} \\ \nr 
	\text{(Lemma 6.4 of \cite{oyrs15})} \leq&  \normlr{\Pi_{\cC_0} \bigg(\ddelta_0^{(t)} + \mu_0 \sum_{g = 1}^{G}   \X_g^T \Big(\oomega_g - \X_g (\ddelta_0^{(t)} + \ddelta_g^{(t)}) \Big) \bigg)}{2} \\ \nr 
	\text{(Lemma 6.2 of \cite{oyrs15})} \leq&   \sup_{\v \in \cB_0 } \v^T \bigg(\ddelta_0^{(t)} + \mu_0 \sum_{g = 1}^{G}   \X_g^T \Big(\oomega_g - \X_g (\ddelta_0^{(t)} + \ddelta_g^{(t)}) \Big) \bigg)%, \quad \cB_0 =  \cC_0 \cap \ball 
	\\ \nr
	\leq&  \sup_{\v \in \cB_0} \v^T \big(\I - \mu_0 \sum_{g = 1}^{G}   \X_g^T\X_g  \big) \ddelta_0^{(t)} +  \mu_0 \sup_{\v \in \cB_0} \v^T \sum_{g = 1}^{G}   \X_g^T \oomega_g 
	\\ \nr 
	+&  \mu_0 \sup_{\v \in \cB_0}  -\v^T \sum_{g=1}^{G}   \X_g^T \X_g \ddelta_g^{(t)}
	\\ \nr 
	\leq&  \norm{\ddelta_0^{(t)}}{2} \sup_{\u, \v \in \cB_0} \v^T \big(\I - \mu_0 \X_0^T\X_0  \big) \u  +  \mu_0 \sup_{\v \in \cB_0} \v^T \X_0^T \frac{\oomega_0}{\norm{\oomega_0}{2}} \norm{\oomega_0}{2} 
	\\ \nr 
	+&  \mu_0 \sum_{g=1}^{G}  \sup_{\v_g \in \cB_0, \u_g \in \cB_g} - \v_g^T \X_g^T \X_g \u_g \norm{\ddelta_g^{(t)}}{2} \\ \label{rewrite}
	\leq&  \rho_0(\mu_0) \norm{\ddelta_0^{(t)}}{2}   +  \xi_0(\mu_0) \norm{\oomega_0}{2} +  \mu_0 \sum_{g=1}^{G}  \frac{\phi_g(\mu_g)}{\mu_g} \norm{\ddelta_g^{(t)}}{2} \\ \nr 
	\eea 
	
	To avoid cluttering we drop $\mu_g$ as the arguments.
	Putting together \eqref{eq:optg} and \eqref{rewrite} inequalities we reach to the followings: 
	\be 
	\nr 
	\norm{\ddelta_g^{(t+1)}}{2} &\leq&   \rho_g\norm{\ddelta_g^{(t)}}{2}   +  \xi_g \norm{\oomega_g}{2} + \phi_g \norm{\ddelta_0^{(t)}}{2} 
	\\ \nr 
	\norm{\ddelta_0^{(t+1)}}{2} &\leq& \rho_0 \norm{\ddelta_0^{(t)}}{2} + \xi_0 \norm{\oomega_0}{2} + \mu_0 \sum_{g=1}^{G}  \frac{\phi_g}{\mu_g} \norm{\ddelta_g^{(t)}}{2}  
	\ee 
\end{IEEEproof}

\subsection{Proof of Lemma \ref{lemm:hpub}}
We will need the following lemma in our proof. 
It establishes the RE condition for individual isotropic sub-Gaussian designs and provides us with the essential tool for proving high probability bounds.  
\begin{lemma}[Theorem 11 of \cite{banerjee14}]
	\label{lem:gennips}
	%To unify the illustration assume, $n_0 = n$ and $\X_0 = \oomega$.
	For all $g \in [G]$, for the matrix $\X_g \in \reals^{n_g \times p}$ with independent isotropic sub-Gaussian rows, i.e., $\normth{\x_{gi}}{\psi_2} \leq k_x$ and $\ex[\x_{gi} \x_{gi}^T] = \I$, the following result holds with probability at least $1 - 2\exp\left( -\gamma_g (\omega(\cA_g) + \tau)^2  \right)$ for $\tau > 0$:
	\be 
	\nr 
	\forall \u_g \in \cC_g: n_g \left(1 -  c_g\frac{\omega(\cA_g) + \tau}{\sqrt{n_g}}\right) \norm{\u_g}{2}^2  \leq \norm{\X_g\u_g}{2}^2 \leq n_g \left(1 +  c_g\frac{\omega(\cA_g) + \tau}{\sqrt{n_g}}\right) \norm{\u_g}{2}^2
	\ee 
	where $c_g > 0$ is constant.% and $(x)_+ = \max(x, 0)$. 
\end{lemma} 

The statement of Lemma \ref{lem:gennips} characterizes the distortion in the Euclidean distance between points $\u_g \in \cC_g$ when the matrix $\X_g/n_g$ is applied to them and states that any sub-Gaussian design matrix is approximately isometry, with high probability:
\be 
\nr 
(1 -  \alpha) \norm{\u_g}{2}^2 \leq \frac{1}{n_g}\norm{\X_g\u_g}{2}^2 \leq (1 + \alpha) \norm{\u_g}{2}^2
\ee 
where $\alpha = c_g \frac{\omega(\cA_g)}{\sqrt{n_g}}$.
Now the proof for Lemma \ref{lemm:hpub}: 
\subsubsection{Bounding $\rho_g(\mu_g)$}

\begin{IEEEproof}
	First we upper bound each of the coefficients $\forall  g \in [G]$:
	\be 
	\nr 
	\rho_g(\mu_g) &=& \sup_{\u, \v \in \cB_g} \v^T \big(\I_g - \mu_g \X_g^T \X_g\big) \u  \nr 
	\ee
	
	We upper bound the argument of the $\sup$ as follows:	
	\be 
	\nr 
	\v^T \big(\I_g - \mu_g \X_g^T \X_g\big) \u 
	&=& \frac{1}{4}\left[(\u + \v)^T(\I - \mu_g \X_g^T \X_g) (\u + \v) - (\u - \v)^T(\I - \mu_g \X_g^T \X_g) (\u - \v) \right] \\ \nr 
	&=& \frac{1}{4}\left[\norm{\u + \v}{2}^2 - \mu_g \norm{\X_g(\u + \v)}{2}^2 - \norm{\u - \v}{2}^2 + \mu_g \norm{\X_g(\u - \v)}{2}^2 \right] \\ \nr 
	\text{(Lemma \ref{lem:gennips})} &\leq& \frac{1}{4}\Bigg[\left(1 - \mu_g n_g \left(1 -  c_g\frac{2 \omega(\cA_g) + \tau}{\sqrt{n_g}}\right)\right) \norm{\u + \v}{2} \\ \nr 
	&-& \left(1 - \mu_g n_g \left(1 +  c_g\frac{2 \omega(\cA_g) + \tau}{\sqrt{n_g}}\right)\right) \norm{\u - \v}{2} \Bigg]\\ \nr 
	\\ \nr 
	\left(\mu_g = \frac{1}{a_g n_g}\right) &\leq& \frac{1}{4}\Bigg[\left(1 - \frac{1}{a_g} \right) \left(\norm{\u + \v}{2}  - \norm{\u - \v}{2} \right) +   c_g\frac{2 \omega(\cA_g) + \tau}{a_g \sqrt{n_g}} \left(\norm{\u + \v}{2} + \norm{\u - \v}{2} \right) \Bigg]\\ \nr 
	&\leq& \frac{1}{4}\Bigg[\left(1 - \frac{1}{a_g} \right) 2\norm{\v}{2} +   c_g\frac{2 \omega(\cA_g) + \tau}{a_g \sqrt{n_g}} 2\sqrt{2} \Bigg]\\ \nr 
	\ee 
	where the last line follows from the triangle inequality and the fact that $\norm{\u + \v}{2} + \norm{\u - \v}{2} \leq 2\sqrt{2}$ which itself follows from $\norm{\u + \v}{2}^2 + \norm{\u - \v}{2}^2 \leq 4$.
	Note that we applied the Lemma \ref{lem:gennips} for bigger sets of $\cA_g + \cA_g$ and $\cA_g - \cA_g$ where Gaussian width of both of them are upper bounded by $2\omega(\cA_g)$.
	
	The above holds with high probability which is computed as follows. %at least $1 - 2\exp\left( -\gamma_g (\omega(\cA_g) + \tau)^2  \right)$.
%	Now we set :
%	\be 
%	\label{eq:rhoub}
%	\v^T \big(\I_g - \frac{1}{a_g n_g} \X_g^T \X_g\big) \u 
%	&\leq& \frac{1}{2}  \left[\left(1 - \frac{1}{a_g} \right) + \sqrt{2} c_g\frac{2 \omega(\cA_g) + \tau}{a_g \sqrt{n_g}} \right]
%	\ee 
%	Now we rewrite the same analysis using the tail bounds for the coefficients to clarify the probabilities. 
	Let's set $\mu_g = \frac{1}{a_g n_g}$, $d_g := \frac{1}{2}\left(1 - \frac{1}{a_g} \right) + \sqrt{2} c_g\frac{\omega(\cA_g) + \tau/2}{a_g \sqrt{n_g}}$ and name the bad events of $\norm{\X_g(\u + \v)}{2}^2 < n_g \left(1 -  c_g\frac{2 \omega(\cA_g) + \tau}{\sqrt{n_g}}\right) $ and $\norm{\X_g(\u - \v)}{2}^2 > n_g \left(1 +  c_g\frac{2 \omega(\cA_g) + \tau}{\sqrt{n_g}}\right)$ as $\cE_1$ and $\cE_2$ respectively. Then from the law of total probability we have:
	\be 
	\nr 
	\pr(\rho_g(\mu_g) \geq d_g) 
	&\leq& \pr(\rho_g(\mu_g) \geq d_g | \neg\cE_1, \neg\cE_2) + \pr(\cE_1, \cE_2)  
	\\ \nr 
	&\leq& 0 + \pr(\cE_1|\cE_2) \pr(\cE_2)   
	\leq \pr(\cE_2)   
	\\ \nr 	
	(\text{Lemma \ref{lem:gennips}}) &\leq& 2\exp\left( -\gamma_g (\omega(\cA_g) + \tau)^2  \right)
	\ee
	which concludes the proof. 	
\end{IEEEproof}
		 
%\subsection{Proof of Proposition Proposition \ref{prop:2}}
%\begin{IEEEproof} 
%	A similar analysis to the proof of Lemma Lemma \ref{lemm:hpub} shows the following bound with probability at least $1 - 6\exp\left( -\gamma_g (\omega(\cA_g) + \tau)^2  \right)$ :
%	\be 
%	\nr 
%	\rho_g\left(\frac{1}{\alpha n_g}\right) \leq 2 c_g\frac{\omega(\cA_g) + \tau}{\sqrt{n_g}}. 
%	\ee
%	for $\alpha > 1$.
%	Note that the bound is twice the case in which $\alpha = 1$, i.e, Lemma Lemma \ref{lemm:hpub}. 
%	Also, Lemma Lemma \ref{lemm:mainlem} readily provides a high probability upper bound for $\eta_g(1/(\alpha n_g))$ as $\sqrt{(2K^2 + 1)}/\alpha \left(\zeta_g k \omega(\cA_g) + \epsilon_g \sqrt{\log G} +  \tau \right)/\sqrt{n_g}$.
%	Replacing $\alpha$ with $G+1$ and redoing the proof of Theorem Theorem \ref{theo:step} completes the proof. 
%\end{IEEEproof}


%\subsection{Proof of Lemma Lemma \ref{lemm:simp}}
%	We simply write the law of total probability:
%	\be 
%	\nr 
%	\pr \left(XY \leq ab \right) &=& \pr (XY \leq ab | X \leq a ) \pr(X \leq a) + \pr (XY \leq ab | X > a ) \pr(X > a) 
%	\\ \nr 
%	&\leq& \pr(X \leq a) + \pr (XY \leq ab | X > a )  
%	\\ \nr 
%	&=& \pr(X \leq a) + \int_{-\infty}^{\infty} \int_{a}^{\infty} \pr(X =  x, Y = y) \1 (XY \leq ab) dx dy   
%	\\ \nr
%	&\leq& \pr(X \leq a) + \int_{-\infty}^{b} \int_{a}^{\infty} \pr(X =  x, Y = y) \1 (XY \leq ab) dx dy 
%	\\ \nr 
%	&+& \int_{b}^{\infty} \int_{a}^{\infty} \pr(X =  x, Y = y) \1 (XY \leq ab) dx dy   
%	\\ \nr
%	(X > a, Y > b \Rightarrow \1(XY \leq ab) = 0)&\leq& \pr(X \leq a) + \int_{-\infty}^{b} \int_{a}^{\infty} \pr(X =  x, Y = y) \1 (XY \leq ab) dx dy 
%	\\ \nr 	
%	&\leq& \pr(X \leq a) + \int_{-\infty}^{b} \int_{a}^{\infty} \pr(X =  x, Y = y) dx dy 
%	\\ \nr 	
%	&\leq& \pr(X \leq a) + \int_{-\infty}^{b} \int_{-\infty}^{\infty} \pr(X =  x, Y = y) dx dy 
%	\\ \nr 	
%	&\leq& \pr(X \leq a) + \pr(Y \leq b)  
%	\ee 
%	We repeat the same procedure to get the other inequality:
%	\be 
%	\nr 
%	\pr \left(X+Y \leq a+b \right) &\leq&  \pr(X \leq a) + \pr(X + Y \leq a + b | X > a)
%	\\ \nr 
%	&\leq&  \pr(X \leq a) + \int_{-\infty}^{\infty} \int_{a}^{\infty} \pr(X =  x, Y = y) \1 (X+Y \leq a+b) dx dy 
%	\\ \nr 
%	&\leq&  \pr(X \leq a) + \int_{-\infty}^{b} \int_{a}^{\infty} \pr(X =  x, Y = y)  dx dy 
%	\\ \nr 
%	&\leq& \pr(X \leq a) + \pr(Y \leq b)  
%	\ee \qed
\subsubsection{Bounding $\eta_g(\mu_g)$}

\begin{IEEEproof}
	The proof of this bound has been worked out during the proof of Lemma \ref{lemm:mainlem} where we show the following in equations \eqref{eq:twoterms} and \eqref{eq:widthbound}
	\[
	\eta_g(\mu_g) = \mu_g \sup_{\v \in \cB_g} \v^T \X_g^T \frac{\w_g}{\norm{\w_g}{2}} = \mu_g c_g k_x (\omega(\cA_g) + \tau), \quad \text{w.p. at least} \quad 1 - \pi_g \exp\left( -\tau^2 \right)
	\]
\end{IEEEproof}

\subsubsection{Bounding $\phi_g(\mu_g)$}
\begin{IEEEproof}
	The following holds for any $\u$ and $\v$ because of $\norm{\X_g (\u + \v)}{2}^2 \geq 0$:
	\be 
	\nr 
	-\v^T \X_g^T \X_g \u \leq \frac{1}{2} \left(\norm{\X_g \u}{2}^2 + \norm{\X_g \v}{2}^2 \right)
	\ee 
	Now we can bound $\phi_g$ as follows:
	\be
	\nr  
	\phi_g(\mu_g) = \mu_g \sup_{\v \in \cB_g, \u \in \cB_0} -\v^T \X_g^T \X_g \u 
	&\leq& \frac{\mu_g}{2} \left(\sup_{\u \in \cB_0} \norm{\X_g \u}{2}^2 + \sup_{\v \in \cB_g} \norm{\X_g \v}{2}^2 \right)
	\ee 
	So we have:
	\be 
	\nr 
	\phi_g\left(\frac{1}{a_g n_g}\right) 
	&\leq& \frac{1}{2a_g} \left(\frac{1}{n_g}\sup_{\u \in \cB_0} \norm{\X_g \u}{2}^2 + \frac{1}{n_g}\sup_{\v \in \cB_g} \norm{\X_g \v}{2}^2 \right) 
	\\ \nr 
	\text{(Lemma \ref{lem:gennips})} &\leq& \frac{1}{a_g}  \left(1 + c_{0g}\frac{\omega(\cA_g) + \omega(\cA_0) + 2 \tau}{2\sqrt{n_g}} \right)
	\\ \nr 
	(\omega_{0g} = \max(\omega(\cA_0), \omega(\cA_g)) &\leq& \frac{1}{a_g}  \left(1 + c_{0g}\frac{\omega_{0g} + 2\tau}{\sqrt{n_g}} \right)
	\ee
	where $c_{0g} = \max(c_0, c_g)$. 
	
	To compute the exact probabilities lets define $s_g := \frac{1}{a_g}  \left(1 + c_{0g}\frac{\omega(\cA_g) + \omega(\cA_0) + 2\tau}{2\sqrt{n_g}} \right)$ and name the bad events of $\frac{1}{n_g}\sup_{\u \in \cB_0} \norm{\X_g \u}{2}^2 > 1 + c_{0}\frac{\omega(\cA_0) + \tau}{\sqrt{n_g}}$ and $\frac{1}{n_g}\sup_{\v \in \cB_g} \norm{\X_g \v}{2}^2 > 1 + c_{g}\frac{\omega(\cA_g) + \tau}{\sqrt{n_g}}$ as $\cE_1$ and $\cE_2$ respectively. Then from the law of total probability we have:
	\be 
	\nr 
	\pr (\phi_g(\mu_g) > s_g) 
	&\leq& \pr (\phi_g(\mu_g) > s_g | \neg \cE_1, \neg \cE_2) + \pr(\cE_1, \cE_2)
	\\ \nr
	&\leq& 0 + \pr(\cE_1| \cE_2) \pr(\cE_2)
%	\\ \nr
	\leq \pr(\cE_2)
	\\ \nr	
	(\text{Lemma \ref{lem:gennips}}) &\leq& 2\exp\left( -\gamma_g (\omega(\cA_g) + \tau)^2 \right)
	\ee
	which concludes the proof.
\end{IEEEproof}


\subsection{Proof of Lemma \ref{paley}}
\begin{IEEEproof}
	To obtain lower bound, we use the Paley--Zygmund inequality for the zero-mean, non-degenerate ($0 < \alpha \leq \ex |\langle \x, \u \rangle|, \u \in \sphere$) sub-Gaussian random vector $\x$ with $\normth{\x}{\psi_2} \leq k_x$ \cite{trop15}. 
	\be 
	\nr 
	Q_{2\xi}(\u)  \geq \frac{(\alpha - 2\xi)^2}{4ck_x^2}.
	\ee 	
\end{IEEEproof}	

\subsection{Proof of Lemma \ref{incolem main}}
\begin{IEEEproof}
	We split $[G]-\cI$ into two groups $\cJ,\cK$. $\cJ$ consists of $\ddelta_g$'s with $\norm{\ddelta_g}{2}\geq 2\norm{\ddelta_0}{2}$ and $\cK=[G]-\cI-\cJ$. We use the bounds
	\[
	\norm{\ddelta_0+\ddelta_g}{2}\geq 
	\begin{cases}
		\lamin(\norm{\ddelta_g}{2}+\norm{\ddelta_0}{2}) &\text{if}~g\in \cI
		\\ 
		\norm{\ddelta_g}{2}/2 &\text{if}~g\in \cJ
		\\
		0 &\text{if}~g\in \cK			
	\end{cases}
	\] 
	This implies
	\[
	\sum_{g=1}^G n_g\norm{\ddelta_0+\ddelta_g}{2}\geq \sum_{g\in \cJ}\frac{n_g}{2}\norm{\ddelta_g}{2}+\lamin\sum_{g\in \cI} n_g (\norm{\ddelta_g}{2}+\norm{\ddelta_0}{2}).
	\]
	Let $S_\cS=\sum_{g\in \cS}n_g\norm{\ddelta_g}{2}$ for $\cS=\cI,\cJ,\cK$.
	We know that over $\cK$, $\norm{\ddelta_g}{2}\leq 2\norm{\ddelta_0}{2}$ which implies $S_\cK = \sum_{g\in \cK}n_g\norm{\ddelta_g}{2}\leq 2\sum_{g\in \cK}n_g\norm{\ddelta_0}{2}\leq 2n\norm{\ddelta_0}{2}$. Set $\rinc=\min\{1/2,\lamin\ratio/3\}$. %=\lamin\ratio/3$.  
	Using $1/2\geq \rinc$, we write:
	\be 
	\nr 
	\sum_{g=1}^G n_g\norm{\ddelta_0+\ddelta_g}{2}
	&\geq& \rinc S_\cJ +\lamin\sum_{g\in \cI}n_g (\norm{\ddelta_g}{2}+\norm{\ddelta_0}{2})
	\\ \nr 
	(S_\cK \leq 2n\norm{\ddelta_0}{2}) &\geq& \rinc S_\cJ +\rinc S_\cK - 2\rinc n\norm{\ddelta_0}{2}+\left(\sum_{g\in \cI} n_g\right)\lamin \norm{\ddelta_0}{2}+\lamin S_{\Ic}
	\\ \nr 
	(\lamin\geq \rinc) &\geq& \rinc (S_\cI + S_\cJ + S_\cK)+ \left(\left(\sum_{g\in \cI} n_g\right)\lamin-2\rinc n\right)\norm{\ddelta_0}{2}.
	\ee 
	Now, observe that, assumption of the \eqref{incodef}, $\sum_{g\in \cI} n_g \geq \ratio n$ implies:
	\be 
	\nr 
	\left(\sum_{g\in \cI} n_g\right)\lamin-2\rinc n\geq (\ratio\lamin -2\rinc)n\geq \rinc n.
	\ee 
	Combining all, we obtain:
	\be 
	\nr 
	\sum_{g=1}^Gn_g \norm{\ddelta_0+\ddelta_g}{2} \geq \rinc (S_\cI + S_\cJ + S_\cK + \norm{\ddelta_0}{2}) = \rinc(n\norm{\ddelta_0}{2} +\sum_{g=1}^G n_g\norm{\ddelta_g}{2}).
	\ee 
\end{IEEEproof}

==> sec/real.tex <==
\begin{figure}
	\centering
	\begin{subfigure}[b]{0.22\textwidth}
		\includegraphics[width=\textwidth]{./img/dr4.pdf}
		\caption{}\label{fig:dr}
	\end{subfigure} ~
	\begin{subfigure}[b]{0.22\textwidth}
		\includegraphics[height=2.7cm]{./img/Saracatinib.pdf}
		\caption{}\label{fig:Saracatinib}
	\end{subfigure}
	\squeezeup
	\caption{a) A sample fitted dose-response curve where Activity Area $y_{gi}$ is shaded. b) Distribution of responses to Saracatinib for which some lung and blood cancer cell lines have responded.}
	\label{fig syn3}
\end{figure}
\section{Anti-Cancer Drug Sensitivity Prediction}
\label{realexp}
In this section, we investigate the application of \dc{} in analyzing the response of cancer tumor cell lines to different doses of various drugs. 
Each cancer type (lung, blood, etc.) is a group $g$ in our DE model and the respond of patient $i$ with cancer $g$ to the drug is our output $y_{gi}$. 
The set of features for each patient $\x_{gi}$ consists of gene expressions, copy number variation, and mutations and $y_{gi}$ is the ``activity area'' above the dose-response curve, Figure \ref{fig:dr}.
Given $\x_{gi}$ and a drug, we want accurately predict a patient's response to a drug and identifying genetic predictors of drug sensitivity. 
%We present more details about and results of the drug sensitivity experiment in Appendix \ref{?}.
%In other words, we are interested in both predicting of $y_{gi}$ and identifying feature $j$ with highest absolute $\bbeta_{g}(j)$ value for each cancer $g$.
%We hope that the data enriched model captures the important shared feature between cancers, as long as the cancer-specific genetic factors that determine the response to therapy.
%In the following, we first explain the dataset and then compare the prediction performance of DS with elastic net on 24 drugs. 
%Then, we perform a more detailed study of the features selected by DS to validate if DS extracts meaningful feature for each cancer. 
%\subsection{Data Set}
%A dose-response dataset of an anticancer drug $d$ and a cell line $gi$ (sampled from a patient $i$ with cancer $g$) consists of pairs ${(c, p)}$ which means proportion $p$ of cells of the cell line $gi$ are alive (relative viability) when treated with drug $d$ with concentration $c$. 
%%There are many methods that fit different function to dose-response data, 
%When a drug \emph{works}, after fitting a function to raw data, we will have a reverse sigmoid-like graph, e.g., Figure \ref{fig:dr}. 
%An effective drug kills more cells with lower concentrations therefore its  ``activity area'' \cite{zoha05}, i.e., area above the curve in Figure \ref{fig:dr}, is larger.
%%There are many ways to measure the drug efficacy from the dose-response curve. 
%We use the activity area of the drug for cell line $gi$ as our output of interest $y_{gi}$. 
%
%\begin{figure}
%	\centering
%	\includegraphics[width=0.3 \textwidth,]{./img/dr4}
%	\caption{}
%	\label{fig:dr}
%\end{figure}
%\vspace{-3mm}
\begin{table*}[bp]
	\centering
	{\small
		\begin{tabular}{ |c|c|c|c|  }
			\hline 	
			\multicolumn{2}{|c|}{Blood and Lymph} & \multicolumn{2}{c|}{Lung}\\
			\hline
			Highlights &    p-Val  & Highlights &    p-Val   \\
			\hline
			Viral leukemogenesis		 & 6.17E-4  & Primary mucoepidermoid carcinoma of lung & 1.85E-4  \\
			Primary cutaneous marginal zone B-cell lymphoma	 & 1.85E-3   & Lung carcinoma cell type unspecified stage IV	& 1.85E-4   \\
			Burkitt Lymphoma	 & 5.50E-3  & Primary adenocarcinoma of lung  & 1.85E-4 \\
			\hline
		\end{tabular}
		\caption{Highlights of interpretable outcomes of \dc{}. p-Values are computed by  Fisher's exact test \cite{chen09toppgene}.}
		\label{table:1}}
\end{table*}
%In this experiment 
We use Cancer Cell Line Encyclopedia (CCLE) \cite{barretina2012cancer} which is a compilation $\sim$500 human cancer cell lines for 36 cancer types where their responses to 24 anticancer drugs have been measured.%\footnote{Here the technical meaning of response $y_{gi}$ is the ``activity area'' above the dose-response curve\cite{barretina2012cancer}.}.
%The goal of the study was to identify genetic predictor of drug sensitivity for different cancers. 
%The method used for analysis of CCLE in the original paper was Elastic Net \cite{zoha05} which we use as the comparison baseline. 
%\footnote{Cancer type is the first tissue where the cancer was observed.} 
We perform two \emph{experiments} where the number of cancers in each data set are $G =2$ or $3$ and we name them TWO and THREE experiments, respectively. 
We consider lung and blood\footnote{By blood cancer, we mean any cancer originate from haematopoietic and lymphoid tissues.} 
for TWO while for THREE we predict the drug sensitivity of skin, breast and ovary cancer cell lines. 
Beyond these five cancer types, others have less than 50 samples, so we remove them from consideration.
Each experiment consists of 24 \emph{problems} each corresponds to a drug. % drug sensitivity prediction of 
Not all of the $~$500 cell lines have been treated with all of the drugs. 
Therefore each problem has a different number of samples $n$ where $n \in [90, 160]$ for TWO and $n \in [70, 100]$ for THREE experiments.
We perform a standard preprocessing \cite{barretina2012cancer} where we remove features with less than $.2$ absolute correlation with the response.% of interest.% which reduces the dimension from $>30,000$ to $p \in [?, ?]$.% range. 
The features that get removed vary by problem, so the dimension $p$ is reduced from from $>30,000$ to $p \in [1000, 15000]$. 
	\begin{figure}
	\centering
	\begin{subfigure}[b]{0.22\textwidth}
		\includegraphics[width=\textwidth]{./img/lung-blood-barplot.pdf}
		\caption{Lung and Blood}\label{fig:two}
	\end{subfigure} ~
	\begin{subfigure}[b]{0.22\textwidth}
		\includegraphics[width=\textwidth]{./img/skin-ovary-breast.pdf}
		\caption{Skin, Ovary, and Breast}\label{fig:three}
	\end{subfigure}
	\squeezeup
	\caption{Distribution of MSE Comparison of Mean Square Error of \dc{} and BL in predicting the response to 24 drugs in TWO and THREE experiments. Each bar is the mean of MSE for 5-fold cross-validation.}
	\label{fig syn4}
\end{figure}
%\subsection{Results}

{\bf Prediction:} In each TWO and THREE experiments, we predict the drug sensitivity for 24 different drugs using sparse DE estimator \eqref{sde}.  %= \{f_g(\bbeta) < b_g\}$
Since the values of $d_g$  in constraint sets $\Omega_{f_g}(d_g)$  are unknown, we tune them by 5-fold cross-validation and report the mean squared error (MSE) of \dc{} and a baseline method. 
Our \emph{baseline} method BL is the LASSO \cite{tibs96} equivalent of DE where we set $\forall g \in [G]_\setminus d_g = 0$ and only estimate the common parameter $\bbeta_0$. 
Figure \ref{fig:two} and \ref{fig:three} illustrate the performance of \dc{} and BL for both experiments. 
Note that \dc{} outperforms BL in 21 and 18 out of 24 problems in TWO and THREE experiments, respectively.

To ensure that the prediction improvement of \dc{} over the baseline is statistically significant, we supplement our analysis with the bootstrapped error of both methods for the TWO experiment.
For each problem in the TWO experiment, we generate 100 bootstrapped data sets by sampling with replacement as $\{(\X^{(i)}_{\text{TWO}}, \y^{(i)}_{\text{TWO}})\}_{i=1}^{100}$.  
Then, we fix $d_g$s hyper-parameters to values determined by cross-validation in the last stage and run both methods and compute pairs of MSEs as $\{(\text{MSE}^{(i)}_{\text{\dc}}, \text{MSE}^{(i)}_{\text{BL}})\}_{i=1}^{100}$ for each problem (drug). We perform paired t-test to determine if difference between means of two methods' MSEs is significant. In 21 out of 24 problems \dc's MSE is lesser than BL's with significance level of $\alpha = 0.05$. A representative set of results is demonstrated in Figure \ref{fig:allbars}. 

	




	\begin{figure}
	\centering
	\begin{subfigure}[b]{0.22\textwidth}
		\centering
		\includegraphics[width=\textwidth]{./img/bar1.pdf}
		\caption{}    
%		\label{fig:mean and std of net14}
	\end{subfigure}
	\hfill
	\begin{subfigure}[b]{0.22\textwidth}  
		\centering 
		\includegraphics[width=\textwidth]{./img/bar2.pdf}
		\caption{}    
%		\label{fig:mean and std of net14}
	\end{subfigure}
	\vskip\baselineskip
	\begin{subfigure}[b]{0.22\textwidth}   
		\centering 
		\includegraphics[width=\textwidth]{./img/bar3.pdf}
		\caption{}    
%		\label{fig:mean and std of net14}
	\end{subfigure}
	\quad
	\begin{subfigure}[b]{0.22\textwidth}   
		\centering 
		\includegraphics[width=\textwidth]{./img/bar4}
		\caption{}    
%		\label{fig:mean and std of net14}
	\end{subfigure}
	\squeezeup
	\caption{MSE for 100 bootstrapped dataset of four drugs of experiment TWO. (a),(b) Sample result of large difference between mean of MSEs and small p-values. (c) Smaller mean difference with significant p-value. (d) One of the three cases where \dc{} is outperformed by the baseline.} 
	\label{fig:allbars}
	\end{figure}


{\bf Interpretation}
%Next we focus on the interpretation of the selected genes. 
We select Saracatinib, a drug which shows activity on both lung and blood cancer cell lines, Figure \ref{fig:Saracatinib}. 
Then, during the bootstrap experiment on TWO, we record support of the estimated parameters by \dc. 
%Fixing the $d_g$ parameters, 
We pick the top five most frequently selected genes across 100 bootstrapped runs for further analysis. 
Now, we have three lists of genes for common, lung , and blood parameters. 
We perform gene enrichment analysis using ToppGene \cite{chen09toppgene} to see where in functional/disease/drug databases these genes have been observed together with statistical significance. 
Table \ref{table:1} summarizes a highlight of our findings which shows lung and blood parameters' supports are capturing a meaningful set of genes as a biomarkers.% for anticancer drug sensitivity.% while the shared parameter has mixed set of genes. 
%{\small 
%\begin{tabular}{ |c|c|c|c|c|c|  }
%	\hline 	
%	\multicolumn{2}{|c|}{(Blood, 512)} & \multicolumn{2}{c|}{(Lung, 500)} & \multicolumn{2}{c|}{(Shared, 525)}\\
%	\hline
%	Highlights &    p-Val  & Highlights &    p-Val &  Highlights &    p-Val \\
%	\hline
%	regulation of immune response	 & 2.1E-8  & Secondary malignant neoplasm of lung & 8.9E-6  &  Acute	Myeloid Leukemia & 5.0E-7 \\
%	T cell activation	 & 5.0E-8   & Lung Cancer  & 2.9E-5  &  Chronic Myeloid Leukemia & 3.0E-5 \\
%	leukocyte activation & 1.0E-6  & Adenosquamous cell lung cancer	 & 3.9E-5  &  Adenocarcinoma of lung & 4.8E-5 \\
%	\hline
%\end{tabular}
%}

%{ (Type, $|\text{supp}(\cdot)|$)} 	&   , ; 2.907E-5  & asd;flkajsdf ;as  &  asdf'alsdkfad' \\
%&   , stage IV;   & asd;flkajsdf ;as  &  asdf'alsdkfad' \\
